Distributed Global Structure-from-Motion with a Deep Front-End

While initial approaches to Structure-from-Motion (SfM) revolved around both global and incremental methods, most recent applications rely on incremental systems to estimate camera poses due to their superior robustness. Though there has been tremendous progress in SfM `front-ends' powered by deep models learned from data, the state-of-the-art (incremental) SfM pipelines still rely on classical SIFT features, developed in 2004. In this work, we investigate whether leveraging the developments in feature extraction and matching helps global SfM perform on par with the SOTA incremental SfM approach (COLMAP). To do so, we design a modular SfM framework that allows us to easily combine developments in different stages of the SfM pipeline. Our experiments show that while developments in deep-learning based two-view correspondence estimation do translate to improvements in point density for scenes reconstructed with global SfM, none of them outperform SIFT when comparing with incremental SfM results on a range of datasets. Our SfM system is designed from the ground up to leverage distributed computation, enabling us to parallelize computation on multiple machines and scale to large scenes.

==> figures/fig-frontend_arch.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/gtsfm - correspondence generator.pdf}
    \caption{The different possible configurations for the global SfM frontend. (a) + (c): detector, descriptor, matcher, (b)+(c): joint detector and describer followed by matcher, (d) end-to-end joint detector matcher.}
    \label{fig:frontend-arch}
\end{figure}

==> figures/sfm_results.tex <==
\begin{tabular}{l r rrr r rrr r rrr r rrr r rrr r rrr}
\toprule
    & \textbf{\# Images}    &  \multicolumn{3}{c}{\textbf{\# Registered}}   &&   \multicolumn{3}{c}{\textbf{\# Points} (Avg. Track Length)}  &&   \multicolumn{3}{c}{\textbf{Time [s]}} &&   \multicolumn{3}{c}{\textbf{Avg. Reproj. Error [px]}}     && \multicolumn{3}{c}{\textbf{Reconstruction Metric?}} && \multicolumn{3}{c}{\textbf{Pose AUC} (@$5^\circ$/@$10^\circ$/@$20^\circ$)} \\
\cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-13}\cmidrule{15-17}\cmidrule{19-21} \cmidrule{23-25}
        &          & COLMAP & Theia & Ours && COLMAP & Theia & Ours && COLMAP & Theia & Ours && COLMAP & Theia & Ours && COLMAP & Theia & Ours && COLMAP & Theia & Ours \\
\midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \multicolumn{25}{l}{DisCO~\cite{crandall2011discrete}} \\
 Rome   & 74,394   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && --- & --- & --- && --- & --- & --- \\
 Quad   &  6,514   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && --- & --- & --- && --- & --- & --- \\
 \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[gray]{0.9} 
 \multicolumn{25}{l}{1DSfM~\cite{wilson2014robust}} \\
\rowcolor[gray]{0.9} 
 Alamo   & 2,915   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && --- & --- & --- && --- & --- & --- \\
\rowcolor[gray]{0.9} 
 Madrid Metropolis   & 1,344   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && --- & --- & --- && --- & --- & --- \\
\rowcolor[gray]{0.9} 
 Montreal Notre Dame   & 2,298   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && --- & --- & --- && --- & --- & --- \\
\rowcolor[gray]{0.9} 
 $\cdots$   &    &  &  &  &&  &  &  &&  &  &  &&  &  &  &&  &  & &&  &  &  \\
 \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \multicolumn{25}{l}{Tanks \& Temples~\cite{knapitsch2017tanks}} \\
 Church   & 507   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD \\
 Courthouse   & 1,106   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD \\
 $\cdots$   &    &  &  &  &&  &  &  &&  &  &  &&  &  &  &&  &  & &&  &  &  \\
 \midrule %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[gray]{0.9} 
 \multicolumn{25}{l}{AstroVision~\cite{driver2023astrovision}} \\
\rowcolor[gray]{0.9} 
 Dawn @ 1 Ceres   & TBD   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD \\
\rowcolor[gray]{0.9} 
 Dawn @ 4 Vesta   & TBD   & TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD && TBD & TBD & TBD \\
\rowcolor[gray]{0.9} 
 $\cdots$   &    &  &  &  &&  &  &  &&  &  &  &&  &  &  &&  &  & &&  &  &  \\
\bottomrule
\end{tabular}



==> tex/accuracy_table_v1.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=\linewidth}
\begingroup
\begin{tabular}{lllllllllllllllllllllllll}
\toprule
\rowcolorize Dataset    & Front-End & \# input & \# Retrieved & Front-End    & Front-End     & Front-End  & VG       & VG        & VG         & VG inlier  & VG inlier  & RA           & TA          & \# Reg. & BA         & BA         & BA            & BA           & BA          & BA     & BA        & BA      & BA       & BA       \\
\rowcolorize           &           & images   & image        & Rot. angular & Trans.        & Pose       & \# input & \# inlier & \# outlier & Rot        & trans.     & rot.         & trans.      & Cameras & \# Tracks  & track      & reproj        & rot.         & trans.      & Pose   & Pose      & Pose    & Pose     & Pose     \\
\rowcolorize           &           &          & pairs        & errors       & Angular       & Errors     & edges    & edges     & edges      & angular    & angular    & angular      & angle       &         & (filtered) & lengths    & errors        & angle        & angle       & AUC    & AUC       & AUC     & AUC      & AUC      \\
\rowcolorize           &           &          &              & (deg.)       & errors (deg). & (deg.)     &          &           &            & errors deg & errors deg & error (deg)  & error (deg) &         &            & (filtered) & filtered (px) & error (deg)  & error (deg) & @1 deg & @2.5 deg. & @5 deg. & @10 deg. & @20 deg. \\
 \midrule
RC3        & LightGlue & 65       & 608          & 2.2 / 25.3   & 1.1 / 16.2    & 2.2 / 31.3 & 317      & 300       & 17         & 1.4 / 2.0  & 0.7 / 2.7  & 1.2 / 1.3    & 1.0 / 1.2   & 65      & 3348       & 3 / 4.2    & 0.4 / 0.5     & 0.2 / 0.3    & 0.2 / 0.3   & 73.8   & 88.1      & 93.3    & 96.9     & 98.4     \\
           & LoFTR     & 65       & 608          & 6.7 / 49.8   & 3.9 / 37.6    & 8.7 / 60.5 & 178      & 126       & 52         & 1.4 / 4.3  & 1.1 / 9.4  & 69.0 / 85.6  & 69.1 / 71.0 & 39      & 33939      & 2 / 2.3    & 0.2 / 0.3     & 0.5 / 2.1    & 1.3 / 2.4   & 9.0    & 27.1      & 40.2    & 48.4     & 53.4     \\
           & SIFT      & 65       & 608          & 1.3 / 22.0   & 0.7 / 15.1    & 1.3 / 26.2 & 260      & 247       & 13         & 1.0 / 1.4  & 0.5 / 2.9  & 0.8 / 1.1    & 0.6 / 0.8   & 65      & 18190      & 3 / 3.7    & 0.1 / 0.1     & 0.2 / 0.3    & 0.2 / 0.4   & 72.6   & 86.9      & 92.8    & 96.4     & 98.2     \\
           & SuperGlue & 65       & 608          & 1.9 / 26.6   & 1.0 / 18.7    & 1.9 / 34.4 & 325      & 264       & 61         & 1.2 / 1.7  & 0.6 / 2.2  & 1.1 / 1.2    & 0.7 / 0.9   & 64      & 3369       & 3 / 4.3    & 0.4 / 0.5     & 0.1 / 0.1    & 0.1 / 0.1   & 85.5   & 93.3      & 95.9    & 97.2     & 97.8     \\
% hline
\rowcolorize Ecole      & LightGlue & 35       & 270          & 0.1 / 0.2    & 0.2 / 0.7     & 0.3 / 0.7  & 240      & 240       & 0          & 0.1 / 0.2  & 0.2 / 0.3  & 0.1 / 0.1    & 0.0 / 0.1   & 26      & 3598       & 3 / 4.9    & 0.5 / 0.6     & 0.0 / 0.0    & 0.0 / 0.0   & 71.2   & 73.0      & 73.7    & 74.0     & 74.1     \\
\rowcolorize Superieure & LoFTR     & 35       & 270          & 0.2 / 0.3    & 0.3 / 1.8     & 0.4 / 1.9  & 240      & 240       & 0          & 0.2 / 0.3  & 0.3 / 1.8  & 0.1 / 0.2    & 0.1 / 0.1   & 26      & 24026      & 2 / 2.4    & 0.2 / 0.3     & 0.1 / 0.2    & 0.0 / 0.1   & 59.3   & 67.9      & 71.1    & 72.7     & 73.5     \\
\rowcolorize de Guerre  & SIFT      & 35       & 270          & 0.2 / 0.3    & 0.5 / 0.6     & 0.5 / 0.6  & 268      & 268       & 0          & 0.2 / 0.3  & 0.5 / 0.6  & 0.1 / 0.2    & 0.1 / 2.9   & 35      & 24147      & 3 / 4.0    & 0.2 / 0.2     & 0.0 / 0.1    & 0.1 / 2.8   & 83.8   & 90.0      & 93.6    & 95.4     & 96.3     \\
\rowcolorize           & SuperGlue & 35       & 270          & 0.1 / 0.2    & 0.2 / 0.7     & 0.3 / 0.7  & 241      & 241       & 0          & 0.1 / 0.2  & 0.2 / 0.7  & 0.1 / 0.1    & 0.0 / 0.1   & 26      & 3524       & 3 / 4.9    & 0.5 / 0.6     & 0.0 / 0.0    & 0.0 / 0.0   & 71.0   & 73.0      & 73.6    & 74.0     & 74.1     \\
% hline
Gerrard    & LightGlue & 98       & 723          & 1.6 / 5.0    & 1.2 / 5.6     & 1.9 / 7.0  & 687      & 668       & 19         & 1.5 / 1.7  & 1.1 / 1.5  & 1.8 / 2.0    & 1.0 / 1.1   & 98      & 32309      & 2 / 3.1    & 0.6 / 0.7     & 1.4 / 1.8    & 0.5 / 0.8   & 9.6    & 38.9      & 65.0    & 82.5     & 91.2     \\
Hall       & LoFTR     & 98       & 723          & 2.1 / 10.2   & 1.7 / 20.5    & 2.4 / 21.5 & 613      & 454       & 159        & 1.4 / 1.7  & 1.2 / 1.6  & 3.6 / 3.5    & 2.1 / 2.9   & 94      & 76095      & 2 / 2.3    & 0.3 / 0.4     & 4.1 / 4.0    & 1.6 / 2.4   & 1.5    & 10.9      & 27.7    & 57.0     & 76.3     \\
           & SIFT      & 98       & 723          & 1.5 / 3.2    & 1.4 / 5.9     & 1.9 / 6.5  & 575      & 557       & 18         & 1.3 / 1.7  & 1.4 / 2.3  & 3.4 / 3.4    & 1.4 / 1.8   & 98      & 27832      & 2 / 3.3    & 0.4 / 0.5     & 2.6 / 2.9    & 1.4 / 1.5   & 3.3    & 18.5      & 43.9    & 71.0     & 85.5     \\
           & SuperGlue & 98       & 723          & 1.4 / 3.8    & 1.1 / 4.2     & 1.8 / 5.3  & 682      & 668       & 14         & 1.4 / 1.6  & 1.1 / 1.4  & 1.9 / 2.1    & 0.8 / 0.9   & 98      & 32115      & 2 / 3.1    & 0.6 / 0.7     & 1.4 / 1.7    & 0.5 / 0.7   & 9.9    & 39.8      & 66.5    & 83.2     & 91.6     \\
% hline
\rowcolorize Kings      & LightGlue & 328      & 4495         & 0.4 / 3.3    & 1.9 / 24.3    & 1.9 / 25.3 & 4055     & 4009      & 46         & 0.3 / 0.8  & 1.7 / 22.1 & 0.8 / 0.9    & 0.5 / 1.4   & 327     & 18351      & 2 / 4.1    & 0.5 / 0.6     & 0.1 / 0.2    & 0.2 / 1.0   & 59.6   & 77.8      & 86.6    & 92.4     & 95.7     \\
\rowcolorize College    & LoFTR     & 328      & 4495         & 0.4 / 4.7    & 1.7 / 17.2    & 1.7 / 18.8 & 2952     & 2864      & 88         & 0.4 / 0.8  & 1.5 / 11.2 & 1.0 / 1.1    & 0.3 / 2.7   & 327     & 236481     & 2 / 2.8    & 0.3 / 0.5     & 0.2 / 0.3    & 0.2 / 1.1   & 52.8   & 74.6      & 85.1    & 91.4     & 95.1     \\
\rowcolorize Cambridge  & SIFT      & 328      & 4495         & 0.4 / 1.4    & 2.3 / 21.4    & 2.3 / 21.6 & 3871     & 3846      & 25         & 0.4 / 0.7  & 2.2 / 20.3 & 0.9 / 0.9    & 0.5 / 2.0   & 327     & 35977      & 2 / 2.9    & 1.3 / 1.4     & 0.4 / 0.4    & 0.2 / 1.5   & 36.6   & 65.1      & 79.1    & 87.8     & 93.1     \\
\rowcolorize           & SuperGlue & 328      & 4495         & 0.4 / 3.4    & 1.9 / 25.5    & 1.9 / 26.6 & 4083     & 4024      & 59         & 0.3 / 0.8  & 1.7 / 23.0 & 0.7 / 0.8    & 0.4 / 1.5   & 327     & 17530      & 2 / 4.0    & 0.6 / 0.7     & 0.3 / 0.3    & 0.3 / 1.3   & 45.4   & 69.8      & 81.8    & 89.5     & 94.0     \\
% hline
Palace     & LightGlue & 281      & 2811         & 0.1 / 1.5    & 0.9 / 8.5     & 0.9 / 9.2  & 2781     & 2781      & 0          & 0.1 / 1.0  & 0.9 / 8.2  & 7.7 / 8.0    & 3.2 / 5.8   & 281     & 14608      & 2 / 3.3    & 0.6 / 0.7     & 8.1 / 8.0    & 3.1 / 6.1   & 0.0    & 0.0       & 5.6     & 25.5     & 50.7     \\
of Fine    & LoFTR     & 281      & 2811         & 0.4 / 4.8    & 3.0 / 20.4    & 3.0 / 21.9 & 2754     & 2741      & 13         & 0.4 / 2.1  & 2.9 / 19.0 & 17.7 / 15.3  & 10.1 / 13.4 & 281     & 90492      & 2 / 2.3    & 0.5 / 0.7     & 17.7 / 15.3  & 10.6 / 12.0 & 0.0    & 0.0       & 0.2     & 3.6      & 19.8     \\
Arts       & SIFT      & 281      & 2811         & 0.1 / 0.4    & 0.9 / 3.9     & 0.9 / 4.0  & 2750     & 2744      & 6          & 0.1 / 0.3  & 0.9 / 3.8  & 0.4 / 0.5    & 0.1 / 0.7   & 281     & 101386     & 3 / 5.3    & 0.2 / 0.3     & 0.2 / 0.2    & 0.1 / 0.5   & 76.9   & 90.1      & 94.9    & 97.3     & 98.5     \\
           & SuperGlue & 281      & 2811         & 0.1 / 1.6    & 0.9 / 8.0     & 0.9 / 8.7  & 2776     & 2776      & 0          & 0.1 / 1.0  & 0.9 / 7.6  & 7.6 / 8.1    & 2.5 / 5.5   & 281     & 16506      & 2 / 3.6    & 0.5 / 0.6     & 6.5 / 7.0    & 3.1 / 4.0   & 0.0    & 0.2       & 7.7     & 34.6     & 61.2     \\
% hline
\rowcolorize Skansen    & LightGlue & 131      & 1366         & 0.3 / 2.7    & 1.1 / 10.7    & 1.2 / 11.7 & 1314     & 1312      & 2          & 0.3 / 0.9  & 1.1 / 9.6  & 6.2 / 6.8    & 2.9 / 8.1   & 131     & 13807      & 2 / 3.9    & 0.6 / 0.7     & 4.2 / 4.6    & 1.7 / 6.5   & 0.0    & 1.6       & 11.6    & 45.7     & 69.1     \\
\rowcolorize Kronan-   & LoFTR     & 131      & 1366         & 0.4 / 2.6    & 1.3 / 8.1     & 1.3 / 9.0  & 1181     & 1168      & 13         & 0.4 / 0.6  & 1.2 / 6.0  & 0.3 / 0.4    & 0.3 / 1.9   & 131     & 70681      & 2 / 2.6    & 0.4 / 0.5     & 0.1 / 0.2    & 0.2 / 1.7   & 67.7   & 83.8      & 90.0    & 93.8     & 96.1     \\
\rowcolorize Gothenburg & SIFT      & 131      & 1366         & 0.3 / 1.7    & 1.2 / 9.6     & 1.2 / 10.5 & 1295     & 1293      & 2          & 0.3 / 0.6  & 1.1 / 9.1  & 0.3 / 0.4    & 0.3 / 1.5   & 131     & 37964      & 4 / 7.3    & 0.3 / 0.3     & 0.0 / 0.1    & 0.0 / 0.9   & 86.8   & 93.4      & 95.9    & 97.5     & 98.4     \\
\rowcolorize           & SuperGlue & 131      & 1366         & 0.3 / 1.4    & 1.1 / 9.6     & 1.1 / 9.9  & 1314     & 1314      & 0          & 0.3 / 0.5  & 1.1 / 9.0  & 0.4 / 0.4    & 0.4 / 1.7   & 131     & 14133      & 2 / 5.0    & 0.6 / 0.7     & 0.1 / 0.1    & 0.1 / 1.1   & 75.1   & 87.6      & 92.7    & 95.6     & 97.0     \\
% hline
Skydio     & LightGlue & 500      & 5330         & 0.9 / 11.6   & 1.7 / 23.5    & 1.9 / 27.2 & 4437     & 4253      & 184        & 0.8 / 6.8  & 1.4 / 15.7 & 101.4 / 93.7 & 95.6 / 91.3 & 500     & 79174      & 2 / 2.3    & 0.7 / 0.9     & 102.0 / 93.3 & 95.6 / 91.3 & 0.0    & 0.0       & 0.0     & 0.0      & 0.1      \\
Crane      & LoFTR     & 500      & 5330         & 1.1 / 3.6    & 2.1 / 24.5    & 2.3 / 25.1 & 3585     & 3420      & 165        & 0.9 / 1.9  & 1.7 / 18.3 & 1.4 / 2.6    & 16.1 / 18.7 & 497     & 165541     & 2 / 2.2    & 0.7 / 0.9     & 1.3 / 2.4    & 14.5 / 18.2 & 0.0    & 0.2       & 4.8     & 16.6     & 33.8     \\
Mast       & SIFT      & 500      & 5330         & 1.3 / 2.9    & 3.7 / 32.1    & 3.9 / 32.4 & 3338     & 3175      & 163        & 1.1 / 2.0  & 3.0 / 27.9 & 4.2 / 4.2    & 4.5 / 6.3   & 495     & 56848      & 2 / 2.5    & 0.6 / 0.8     & 3.9 / 3.6    & 2.0 / 4.1   & 0.1    & 2.3       & 19.2    & 50.3     & 72.0     \\
           & SuperGlue & 500      & 5330         & 0.9 / 11.2   & 1.6 / 24.6    & 1.9 / 28.2 & 4424     & 4224      & 200        & 0.8 / 7.2  & 1.4 / 16.4 & 75.7 / 83.7  & 93.1 / 90.5 & 500     & 82205      & 2 / 2.3    & 0.5 / 0.7     & 78.3 / 85.0  & 93.2 / 90.5 & 0.0    & 0.0       & 0.0     & 0.0      & 0.0      \\
% hline
\rowcolorize South      & LightGlue & 128      & 1163         & 0.4 / 8.3    & 0.5 / 6.2     & 0.6 / 9.7  & 1082     & 1055      & 27         & 0.4 / 3.6  & 0.4 / 3.3  & 21.6 / 22.9  & 14.1 / 17.1 & 128     & 21809      & 2 / 2.6    & 0.4 / 0.6     & 13.7 / 13.0  & 7.8 / 9.3   & 0.0    & 0.0       & 0.7     & 4.5      & 31.8     \\
\rowcolorize Building   & LoFTR     & 128      & 1163         & 0.3 / 4.0    & 0.5 / 5.1     & 0.6 / 6.0  & 907      & 898       & 9          & 0.3 / 0.7  & 0.4 / 0.8  & 2.1 / 2.4    & 1.0 / 1.4   & 128     & 175669     & 2 / 2.9    & 0.3 / 0.4     & 0.5 / 0.5    & 0.2 / 0.2   & 50.8   & 80.3      & 90.2    & 95.1     & 97.5     \\
\rowcolorize           & SIFT      & 128      & 1163         & 0.4 / 1.3    & 0.7 / 1.5     & 0.8 / 1.8  & 828      & 827       & 1          & 0.4 / 0.8  & 0.7 / 1.1  & 1.4 / 1.3    & 0.6 / 0.6   & 128     & 47164      & 2 / 3.4    & 0.2 / 0.3     & 0.6 / 0.6    & 0.3 / 0.3   & 43.3   & 77.3      & 88.7    & 94.3     & 97.2     \\
\rowcolorize           & SuperGlue & 128      & 1163         & 0.4 / 8.3    & 0.4 / 7.0     & 0.6 / 10.2 & 1089     & 1065      & 24         & 0.4 / 4.1  & 0.4 / 4.1  & 23.4 / 20.8  & 15.5 / 15.6 & 128     & 21150      & 2 / 2.6    & 0.5 / 0.7     & 16.2 / 14.9  & 10.3 / 11.0 & 0.0    & 0.9       & 3.4     & 8.8      & 26.7    \\
% hline
% Fort       & LightGlue & 27       & 214          & 0.2 / 0.2    & 0.2 / 0.2     & 0.3 / 0.3  & 214      & 214       & 0          & 0.2 / 0.2  & 0.2 / 0.2  & 0.3 / 0.2    & 0.1 / 3.5   & 27      & 5453       & 3 / 4.8    & 0.5 / 0.5     & 0.0 / 0.0    & 0.0 / 3.4   & 92.9   & 94.9      & 95.6    & 96.0     & 96.1     \\
% Channing   & LoFTR     & 27       & 214          & 0.2 / 0.6    & 0.2 / 2.6     & 0.3 / 2.6  & 202      & 202       & 0          & 0.2 / 0.3  & 0.2 / 0.7  & 0.3 / 0.2    & 0.1 / 3.5   & 27      & 20012      & 2 / 2.7    & 0.2 / 0.3     & 0.0 / 0.1    & 0.0 / 3.4   & 88.4   & 93.2      & 94.7    & 95.5     & 95.9     \\
% Gate       & SIFT      & 27       & 214          & 0.1 / 0.2    & 0.2 / 0.2     & 0.2 / 0.3  & 214      & 214       & 0          & 0.1 / 0.2  & 0.2 / 0.2  & 0.2 / 0.2    & 0.0 / 3.4   & 27      & 11168      & 3 / 4.8    & 0.2 / 0.2     & 0.0 / 0.0    & 0.0 / 3.4   & 94.3   & 95.5      & 95.9    & 96.1     & 96.2     \\
% Singapore  & SuperGlue & 27       & 214          & 0.2 / 0.2    & 0.2 / 0.2     & 0.3 / 0.3  & 214      & 214       & 0          & 0.2 / 0.2  & 0.2 / 0.2  & 0.3 / 0.3    & 0.1 / 3.5   & 27      & 5477       & 3 / 4.8    & 0.5 / 0.5     & 0.0 / 0.0    & 0.0 / 3.4   & 92.9   & 94.9      & 95.6    & 96.0     & 96.1     \\
% % hline
% \rowcolorize Nijo       & LightGlue & 19       & 136          & 0.2 / 0.4    & 0.5 / 0.6     & 0.5 / 0.7  & 136      & 136       & 0          & 0.2 / 0.4  & 0.5 / 0.6  & 0.3 / 0.3    & 0.2 / 5.4   & 19      & 4145       & 2 / 3.4    & 0.4 / 0.5     & 0.2 / 0.2    & 0.1 / 5.3   & 65.0   & 76.8      & 83.9    & 89.3     & 92.0     \\
% \rowcolorize Castle     & LoFTR     & 19       & 136          & 0.2 / 0.4    & 0.5 / 0.7     & 0.5 / 0.7  & 132      & 132       & 0          & 0.2 / 0.4  & 0.5 / 0.6  & 0.2 / 0.2    & 0.2 / 5.3   & 19      & 14918      & 2 / 2.4    & 0.2 / 0.3     & 0.1 / 0.1    & 0.1 / 5.3   & 68.6   & 78.7      & 84.5    & 89.6     & 92.2     \\
% \rowcolorize Gate       & SIFT      & 19       & 136          & 0.3 / 1.0    & 0.5 / 1.1     & 0.6 / 1.2  & 135      & 132       & 3          & 0.3 / 0.6  & 0.5 / 0.8  & 0.3 / 0.3    & 0.2 / 5.4   & 19      & 11847      & 2 / 3.3    & 0.2 / 0.3     & 0.1 / 0.1    & 0.0 / 4.9   & 82.4   & 89.8      & 92.3    & 93.5     & 94.1     \\
% \rowcolorize           & SuperGlue & 19       & 136          & 0.2 / 0.3    & 0.5 / 0.6     & 0.5 / 0.6  & 136      & 136       & 0          & 0.2 / 0.3  & 0.5 / 0.6  & 0.2 / 0.2    & 0.2 / 5.4   & 19      & 4301       & 2 / 3.6    & 0.4 / 0.6     & 0.1 / 0.1    & 0.1 / 5.3   & 66.0   & 77.4      & 84.3    & 89.5     & 92.1     \\
\bottomrule
\end{tabular}
\endgroup
\end{adjustbox}
    \caption{Results with 10 retrieval matches, 5 frame lookahead, at 760p. `Median / Mean' statistics are given for 1d distributions.  Abbreviations: View Graph Estimation (VG), Rotation Averaging (RA), Translation Averaging (TA), Bundle Adjustment (BA)}
    \label{tab:my_label}
\end{table*}


==> tex/olsson_data_with_colmap_gt_tab.tex <==
\begin{table*}[t]
\vspace{-5mm}
    \centering
    \begin{adjustbox}{width=\linewidth}
\begingroup
\begin{tabular}{lllllllllllllllllllllllll}
\toprule
\rowcolorize Dataset    & Front-End & \# Input & \# Retrieved & Front-End      & Front-End      & Front-End      & VG           & VG           & VG             & VG inlier      & VG inlier      & RA             & TA             & \# Reg.      & BA           & BA           & BA             & BA             & BA             & BA           & BA           & BA           & BA           & BA           \\
\rowcolorize           &           & Images   & Image        & Rot. angular   & Trans.         & Pose           & \# input     & \# inlier    & \# outlier     & Rot            & trans.         & rot.           & trans.         & Cameras      & \# Tracks    & track        & reproj         & rot.           & trans.         & Pose         & Pose         & Pose         & Pose         & Pose         \\
\rowcolorize           &           &          & Pairs        & errors         & Angular        & Errors         & edges        & edges        & edges          & angular        & angular        & angular        & angle          &              & (filtered)   & lengths      & errors         & angle          & angle          & AUC          & AUC          & AUC          & AUC          & AUC          \\
\rowcolorize           &           &          &              & (deg.)         & errors (deg).  & (deg.)         &              &              &                & errors (deg.)  & errors (deg.)  & error (deg.)   & error (deg.)   &              &              & (filtered)   & filtered (px)  & error (deg)    & error (deg.)   & @1 deg.      & @2.5 deg.    & @5 deg.      & @10 deg.     & @20 deg.     \\
\rowcolorize           &           &          &              & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\uparrow$) & ($\uparrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\uparrow$) & ($\uparrow$) & ($\uparrow$) & ($\downarrow$) & ($\downarrow$) & ($\downarrow$) & ($\uparrow$) & ($\uparrow$) & ($\uparrow$) & ($\uparrow$) & ($\uparrow$) \\
\midrule
\bottomrule
\end{tabular}
\endgroup
\end{adjustbox}
    \caption{Results with 5 retrieval matches, 10 frame lookahead, at 760p resolution. `Median / Mean' statistics are given for 1d distributions.  Abbreviations: View Graph Estimation (VG), Rotation Averaging (RA), Translation Averaging (TA), Bundle Adjustment (BA)}
    \label{tab:acc-olssondata-colmapGT}
\end{table*}
